Reducing multivariate independence testing to two bivariate means comparisons

Testing for independence between two random vectors is a fundamental problem in statistics. It is observed from empirical studies that many existing omnibus consistent tests may not work well for some strongly nonmonotonic and nonlinear relationships. To explore the reasons behind this issue, we novelly transform the multivariate independence testing problem equivalently into checking the equality of two bivariate means. An important observation we made is that the power loss is mainly due to cancellation of positive and negative terms in dependence metrics, making them very close to zero. Motivated by this observation, we propose a class of consistent metrics with a positive integer $\gamma$ that exactly characterize independence. Theoretically, we show that the metrics with even and infinity $\gamma$ can effectively avoid the cancellation, and have high powers under the alternatives that two mean differences offset each other. Since we target at a wide range of dependence scenarios in practice, we further suggest to combine the p-values of test statistics with different $\gamma$'s through the Fisher's method. We illustrate the advantages of our proposed tests through extensive numerical studies.

==> definition1.tex <==
\usepackage{latexsym, amsbsy, amssymb,multirow, epsfig, amsmath}
\usepackage{hyperref}

%--------------------Initialize---------------------%
%\textheight= 9in  \textwidth = 6.5in \topmargin = -1.4cm
%\oddsidemargin = -0.15in \evensidemargin = 0in
\usepackage{natbib,graphicx,setspace,lscape,longtable}
\usepackage{natbib,epsfig,graphicx,algorithm,algorithmic}
%\usepackage[linesnumbered,boxed,ruled,commentsnumbered]{algorithm2e}%%算法包，注意设置所需可选项
\usepackage{amsmath,amsthm,amssymb,color,bm}
\usepackage{xr}
\RequirePackage[mathlines, displaymath]{lineno}
\bibpunct{(}{)}{;}{a}{,}{,}

%\setlength{\textwidth}{6.2in} \setlength{\textheight}{8.75in}
%\setlength{\topmargin}{-0.25in} \setlength{\oddsidemargin}{0.25in}
%\setlength{\evensidemargin}{0.25in}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
%\newtheorem{theorem}{Theorem}
%\newtheorem{lemma}{Lemma}
%\newtheorem{prop}{Proposition}
\baselineskip = 7mm
\parskip = 2.5mm

\newcommand{\csection}[1]
    {\begin{center}
        \stepcounter{section}
        {\bf\large\arabic{section}. #1}
    \end{center}
    \vspace{-0.15 cm}
}

\newcommand{\scsection}[1]
    {\begin{center}
        {\bf\large #1}
    \end{center}
    \vspace{-0.15 cm}
}

\newcommand{\csubsection}[1]{
\vspace{-0.25 cm}
\begin{center}
\stepcounter{subsection}
{\it\arabic{section}.\arabic{subsection}. #1}
\end{center}
\vspace{-0.25 cm}
}

\newcommand{\scsubsection}[1]{
\vspace{-0.25 cm}
\begin{center}
\stepcounter{subsection}
{\it #1}
\end{center}
\vspace{-0.25 cm}
}

\def\beqr{\begin{eqnarray}}
\def\eeqr{\end{eqnarray}}
\def\beqrs{\begin{eqnarray*}}
\def\eeqrs{\end{eqnarray*}}
\def\bep{\begin{prop}}
\def\eep{\end{prop}}

\def\mR{\mathbb{R}}
\def\calA{\mathcal{A}}
\def\calB{\mathcal{B}}
\def\calC{\mathcal{C}}
\def\calD{\mathcal{D}}
\def\calS{\mathcal{S}}
\def\calP{\mathcal{P}}
\def\calM{\mathcal{M}}
\def\calU{\mathcal{U}}
\def\calT{\mathcal{T}}
\def\calF{\mathcal{F}}

\def\calX{\mathcal{X}}
\def\calY{\mathcal{Y}}
\def\calZ{\mathcal{Z}}
\def\calN{\mathcal{N}}
\def\calK{\mathcal{K}}

\newtheorem{Theorem}{Theorem}[section]
\newtheorem{Corollary}{Theorem}[section]
\newtheorem{Lemma}[Theorem]{Lemma}

\def\bias{\mbox{bias}}
\def\pr{\mbox{pr}}
\def\var{\mbox{var}}
\def\cov{\mbox{cov}}
\def\cor{\mbox{cor}}
\def\MSE{\mbox{MSE}}
\def\arcos{\mbox{arcos}}
\def\MDDM{{\rm{MDDM}}}
\def\MDD{{\rm{MDD}^{2}}}
\def\rS{{\rm{S}}}
\def\KS{{\rm{KS}}}
\def\CvM{{\rm{CvM}}}
\def\rZ{{\rm{Z}}}
\def\PCvM{{\rm{PCvM}}}
\def\GJZZ{{\rm{GJZZ}}}
\def\sign{\mbox{sign}}


%\textheight= 9in
%\textwidth = 6.1in
%\evensidemargin = 0in
%\renewcommand{\thefootnote}{\fnsymbol{footnote}}
%
%
%\numberwithin{equation}{section}
%\renewcommand{\baselinestretch}{1.75}


%\bibliographystyle{cheng}
%\renewcommand\refname{REFERENCE}
%\bibliographystyle{refstyle}
%\renewcommand\refname{REFERENCE}


%-------------Li-Ping's Definition-----------------------%
\def\hDash{\bot\!\!\!\bot}
\def\wh{\widehat}
\def\wt{\widetilde}
\def\ba{\mbox{\boldmath$\alpha$}}
\def\bb{\mbox{\boldmath$\beta$}}
\def\bg{\mbox{\boldmath$\gamma$}}
\def\ha{\mbox{$\widehat\ba$}}
\def\hb{\mbox{$\widehat\bb$}}
\def\hg{\mbox{$\widehat\bg$}}
\def\hDash{\bot\!\!\!\bot}


\def\a{{\bf a}}
\def\b{{\bf b}}
\def\A{{\bf A}}
\def\B{{\bf B}}
\def\C{{\bf C}}
\def\D{{\bf D}}
\def\F{{\bf F}}
\def\G{{\bf G}}
%%\def\m{{\bf m}}
\def\J{{\bf J}}
\def\M{{\bf M}}
\def\X{{\bf X}}
\def\x{{\bf x}}
\def\Y{{\bf Y}}
\def\y{{\bf y}}
\def\Z{{\bf Z}}
\def\z{{\bf z}}
\def\u{{\bf u}}
\def\U{{\bf U}}
\def\W{{\bf W}}
\def\s{{\bf s}}
\def\t{{\bf t}}
\def\h{{\bf h}}
\def\k{{\bf k}}
\def\l{{\bf l}}
\def\c{{\bf c}}
\def\d{{\bf d}}
\def\w{{\bf w}}
\def\g{{\bf g}}
\def\I{{\bf I}}
\def\v1{{\bf 1}}
%\def\vz{{\bf 0}}
%\def\beps{{\bm \epsilon}}

\def\bzeta{{\bm \zeta}}
\def\betaa{{\bm \eta}}
\def\bome{{\bm \omega}}
\def\bpi{{\bm \pi}}
\def\bU{{\bm U}}
\def\bh{{\bm h}}
\def\m{{\bm m}}
\def\vz{{\bm 0}}

\newcommand{\trans}{^{\mbox{\tiny{T}}}}
\def\defby{\stackrel{\mbox{\textrm{\tiny def}}}{=}}

\newcommand{\beps}{\mbox{\boldmath $\varepsilon$}}
\newcommand{\bSig}{\mbox{\boldmath $\Sigma$}}
\newcommand{\hSig}{\mbox{$\widehat{\bSig}$}}
\newcommand{\bLam}{\mbox{\boldmath $\Lambda$}}
\newcommand{\bGam}{\mbox{\boldmath $\Gamma$}}
\newcommand{\hLam}{\mbox{$\widehat{\bLam}$}}
\newcommand{\bOmega}{\mbox{\boldmath $\Omega$}}
\newcommand{\bI}{\mbox{\boldmath $I$}}

\newtheorem{defi}{\sc Definition}[section]
\newtheorem{theo}{\bf Theorem}
\newtheorem{lemm}{\sc Lemma}
\newtheorem{prop}{\sc Proposition}
\newtheorem{coll}{\sc Corollary}[theo]
\newtheorem{rema}{\bf Remark}


%--------------------------------------------------------------%


%\headsep 6pt
%\topmargin 0in
%\textheight 8.5in
%\evensidemargin 0.5in
%\oddsidemargin 0.5in
%\textwidth 6in
%\footskip 18pt

\newtheorem{lemma}{Lemma}
\newtheorem{theorem}{Theorem}


\newcommand{\skipline}{\vspace{12pt}}

\newcommand{\Dcov}{{\rm{Dcov}}}
\newcommand{\Pcov}{{\rm{Pcov}}}
\newcommand{\DC}{{{DC}}}
\newcommand{\PC}{{{PC}}}
\newcommand{\dcov}{{\rm{dcov}}}
\newcommand{\dCor}{{\rm{dCor}}}

\newcommand{\mdCov}{{\rm{mdCov}}}
\newcommand{\mdCor}{{\rm{mdCor}}}

\newcommand{\dCov}{{\rm{dCov}}}
\newcommand{\gHSIC}{{\rm{gHSIC}}}
\newcommand{\HHG}{{\rm{HHG}}}
\newcommand{\pCov}{{\rm{pCov}}}
\newcommand{\RpCov}{{\rm{RpCov}}}
\newcommand{\mBKR}{{\rm{mBKR}}}
\newcommand{\mBDY}{{\rm{mBDY}}}
\newcommand{\bCov}{{\rm{bCov}}}
\newcommand{\RdCov}{{\rm{RdCov}}}
\newcommand{\new}{{\rm{new}}}
\newcommand{\IPR}{{\rm{IPR}}}


\newcommand{\SNR}{{\rm{SNR}}}
\newcommand{\ARE}{{\rm{ARE}}}
\newcommand{\diag}{{\rm{diag}}}

%%\newcommand{\D}{\mbox{D}}
\newcommand{\E}{\mbox{E}}
%\newcommand{\F}{\mbox{F}}
\newcommand{\NLS}{\mbox{NLS}}
\newcommand{\GPLSIM}{\mbox{GPLSIM}}
\newcommand{\Known}{\mbox{Known}}
\newcommand{\PS}{\mbox{PS}}
\newcommand{\PR}{\mbox{PR}}
\newcommand{\LS}{\mbox{LS}}
\newcommand{\LSR}{\mbox{LSR}}
\newcommand{\PPR}{\mbox{PPR}}
\newcommand{\SIR}{\mbox{SIR}}
\newcommand{\pHd}{\mbox{pHd}}
\newcommand{\tr}{\mbox{tr}}
\newcommand{\vech}{\mbox{vech}}
\newcommand{\mvz}{\mbox{${\bf z}$}}
\newcommand{\Hessian}{\mbox{${\bf H}$}}

\newcommand{\ang}{{\rm{ang}}}


\newcommand{\yvec}{\mbox{\boldmath $y$}}

\newcommand{\Zvec}{\mbox{\boldmath $Z$}}
\newcommand{\avec}{\mbox{\boldmath $a$}}
\newcommand{\bvec}{\mbox{\boldmath $b$}}
\newcommand{\mvec}{\mbox{\boldmath $m$}}
\newcommand{\svec}{\mbox{\boldmath $s$}}
\newcommand{\tvec}{\mbox{\boldmath $t$}}
\newcommand{\uvec}{\mbox{\boldmath $u$}}
\newcommand{\wvec}{\mbox{\boldmath $w$}}
\newcommand{\gammavec}{\mbox{\boldmath $\gamma$}}
\newcommand{\epsvec}{\mbox{\boldmath $\epsilon$}}
\newcommand{\zetavec}{\mbox{\boldmath $\zeta$}}
\newcommand{\etavec}{\mbox{\boldmath $\eta$}}
\newcommand{\thetavec}{\mbox{\boldmath $\theta$}}
\newcommand{\chivec}{\mbox{\boldmath $\chi$}}
\newcommand{\Covmat}{\mbox{\boldmath $\Sigma$}}
\newcommand{\Bmat}{\mbox{${\bf B}$}}
\newcommand{\norm}{\|}
\newcommand{\calR}{{\mathbb{R}}}
\newcommand{\bnu}{\mbox{\boldmath $\nu$}}

\newcommand{\calH}{{\mathcal{H}}}
\newcommand{\calI}{{\mathcal{I}}}
\newcommand{\calW}{{\mathcal{W}}}

\newcommand{\calV}{{\mathcal{V}}}

\newcommand{\calG}{{G}}

\usepackage{latexsym}
\usepackage{epsfig}
\usepackage{bm}



% 图表环境
\usepackage[small]{caption2}
\usepackage{threeparttable}
\usepackage{dcolumn}
\usepackage{multirow}
\usepackage{booktabs}
%




%\renewcommand{\baselinestretch}{1.75}
%
%\newcommand{\csection}[1]
%{\begin{center}
%		\stepcounter{section}
%		{\bf\large\arabic{section}. #1}
%	\end{center}
%	\vspace{-0.15 cm}}
%\newcommand{\scsection}[1]
%{\begin{center}
%		{\bf\large #1}
%	\end{center}
%	\vspace{-0.15 cm}}
%\newcommand{\csubsection}[1]{
%	\vspace{-0.25 cm}
%	\begin{center}
%		\stepcounter{subsection}
%		{\it\arabic{section}.\arabic{subsection}. #1}
%	\end{center}
%	\vspace{-0.25 cm}}
%\newcommand{\scsubsection}[1]{
%	\vspace{-0.25 cm}
%	\begin{center}
%		\stepcounter{subsection}
%		{\it #1}
%	\end{center}
%	\vspace{-0.25 cm}}
%
%
%
%
%%\usepackage{xr}
%%\externaldocument{其他文件名称，可以引用其他文件中出现的标号} % 例如，
%\usepackage{xr}
%\externaldocument{chap1}
%% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
%%                      																								  %
%%                      					可能需要使用特殊的一些包    			    			 %
%%                      																								  %
%% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
%\RequirePackage[mathlines, displaymath]{lineno}
%\usepackage{natbib}
%\usepackage{latexsym, amsbsy, amssymb,multirow, epsfig, amsmath}
%\usepackage[left=30mm,right=28mm,top=2cm,bottom=2cm]{geometry}
%%\usepackage{amssymb,amsthm,amsmath,mathrsfs,bm,color}
%%\setlength{\textwidth}{6.2in} \setlength{\textheight}{8.75in}
%%\setlength{\topmargin}{-0.25in} \setlength{\oddsidemargin}{0.25in}
%%\setlength{\evensidemargin}{0.25in}
%%\usepackage{hyperref}
%%\baselineskip = 7mm
%%\parskip = 2.5mm
%%
%%\textheight= 9in
%%\textwidth = 6.1in
%%\evensidemargin = 0in
%%
%
%
%% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
%%                      																								  %
%%                      					可能需要使用特殊的命令行    			    			 %
%%                      																								  %
%% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
%\def\beqr{\begin{eqnarray}}
%\def\eeqr{\end{eqnarray}}
%\def\beqrs{\begin{eqnarray*}}
%\def\eeqrs{\end{eqnarray*}}
%
%% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
%%                      																								  %
%%                      					给出比较常用的定理环境定义  	   	   	    			 %
%%                      																								  %
%% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
%\newtheorem{theo}{\bf Theorem}
%\bibliographystyle{refstyle}
%\renewcommand\refname{REFERENCE}
%
%% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
%%                      																								  %
%%                      					给出比较常用的特殊算子定义  		   	    			 %
%%                      																								  %
%% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
%\def\pr{\mbox{pr}}
%\def\cov{\mbox{cov}}
%\def\var{\mbox{var}}
%\def\sign{\mbox{sign}}
%\def\sp{\textrm{span}}
%\def\vecl{\textrm{vecl}}
%
%
%
%% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
%%                      																								  %
%%                      					给出比较常用的特殊符号定义  		   	    			 %
%%                      																								  %
%% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
%\def\mR{\mathbb{R}}
%\def\calA{\mathcal{A}}
%\def\calB{\mathcal{B}}
%\def\calC{\mathcal{C}}
%\def\calD{\mathcal{D}}
%\def\calI{\mathcal{I}}
%\def\calN{\mathcal{N}}
%\def\calS{\mathcal{S}}
%\def\calX{\mathcal{X}}
%\def\calY{\mathcal{Y}}
%\def\calZ{\mathcal{Z}}
%
%
%\def\a{{\bf a}}
%\def\b{{\bf b}}
%\def\c{{\bf c}}
%\def\d{{\bf d}}
%\def\u{{\bf u}}
%\def\v{{\bf v}}
%\def\w{{\bf w}}
%\def\x{{\bf x}}
%\def\y{{\bf y}}
%\def\z{{\bf z}}
%
%\def\A{{\bf A}}
%\def\B{{\bf B}}
%\def\C{{\bf C}}
%\def\D{{\bf D}}
%\def\I{{\bf I}}
%\def\X{{\bf X}}
%\def\Y{{\bf Y}}
%\def\Z{{\bf Z}}
%
%
%\def\ba{\mbox{\boldmath$\alpha$}}
%\def\bb{\mbox{\boldmath$\beta$}}
%\def\bSig{\mbox{\boldmath$\Sigma$}}
%
%% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
%%                      																								  %
%%                      					给出其他一些的特殊算子定义  		   	    			 %
%%                      																								  %
%% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
%\def\defby{\stackrel{\mbox{\textrm{\tiny def}}}{=}}
%\newcommand{\trans}{^{\mbox{\tiny{T}}}}
%\def\hDash{\bot\!\!\!\bot}
%\def\wh{\widehat}
%\def\wt{\widetilde}

